Insights from Verification: Training a Verilog Generation LLM with Reinforcement Learning with Testbench Feedback

Large language models (LLMs) have shown strong performance in Verilog generation from natural language description. However, ensuring the functional correctness of the generated code remains a significant challenge. This paper introduces a method that integrates verification insights from testbench into the training of Verilog generation LLMs, aligning the training with the fundamental goal of hardware design: functional correctness. The main obstacle in using LLMs for Verilog code generation is the lack of sufficient functional verification data, particularly testbenches paired with design specifications and code. To address this problem, we introduce an automatic testbench generation pipeline that decomposes the process and uses feedback from the Verilog compiler simulator (VCS) to reduce hallucination and ensure correctness. We then use the testbench to evaluate the generated codes and collect them for further training, where verification insights are introduced. Our method applies reinforcement learning (RL), specifically direct preference optimization (DPO), to align Verilog code generation with functional correctness by training preference pairs based on testbench outcomes. In evaluations on VerilogEval-Machine, VerilogEval-Human, RTLLM v1.1, RTLLM v2, and VerilogEval v2, our approach consistently outperforms state-of-the-art baselines in generating functionally correct Verilog code. We open source all training code, data, and models at https://anonymous.4open.science/r/VeriPrefer-E88B.

==> figs/overview.tex <==
\begin{figure*}[htbp]
    \centering
    \includegraphics[width=\linewidth]{figs/overview.pdf}
    \caption{Overview of this work. I.) Specification generation: Practical design specifications $\x_i$ are generated by target Verilog code $\y_i$.  II.) Testbench generation: Automated testbenches are built to collect verification insights.  III.) Preference Pairs Collection: The generated code is tested under testbenches, and code that passes more testcases is considered more preferred, denoted as $ \yplus $, while the other is denoted as $ \yminus $.  IV.) Training: 
    $(\x_i, \y_i)$ is used for supervised fine-tuning; $(\x_i, \yplus, \yminus)$ is used for reinforcement learning.  V.) Inference: The policy model generates Verilog code from new specifications without feedback.
    % guan{what are black arrows}; 
    % \guan{what are the block boxes? some function (inference with LLM) or things generated by some function?}
    }
    \label{fig:overview}
\end{figure*}

==> tables/stage_ablation.tex <==
\begin{table}[htbp]
\centering
\caption{Ablation Study on PPO training.}
\begin{threeparttable}
\setlength{\tabcolsep}{2.5pt}
\begin{tabular}{cccccccccc}
\toprule
\multirow{4}{*}{\textbf{Stage}} & \multirow{4}{*}{\begin{tabular}[c]{@{}c@{}}\textbf{Construction} \\ \textbf{Method}\end{tabular}} & \multirow{4}{*}{\textbf{\#Pairs}} & \multicolumn{3}{c}{\textbf{RTLLM v2}} & \multicolumn{3}{c}{\textbf{VerilogEval v2}} \\
\cmidrule(lr){4-6} \cmidrule(lr){7-9}
& & & \multicolumn{3}{c}{\textbf{Function}} & \multicolumn{3}{c}{\textbf{Function}} \\
\cmidrule(lr){4-6} \cmidrule(lr){7-9}
& & & \p${1}$ & \p${5}$ & \p${10}$ & \p${1}$ & \p${5}$ & \p${10}$ \\
\midrule
\textbf{SFT} & & & 49.8 & 62.5 & 66.1 & 47.8 & 64.3 & 69.1 \\
\midrule
\multirow{4}{*}{\textbf{PPO}}
& \textbf{AST} & 4222 & 47.5 & 58.8 & 61.2 & 47.0 & 59.1 & 63.1 \\
& \textbf{DFG} & 2834 & 48.4 & 57.9 & 61.9 & 45.5 & 60.9 & 62.7 \\
& \textbf{BLEU} & 4706 & 48.0 & 57.5 & 63.2 & 46.2 & 60.5 & 61.4 \\
& \textbf{Testbench} & 1796 & 49.3 & 58.4 & 62.1 & 45.4 & 59.4 & 62.1 \\

\bottomrule
\end{tabular}
\label{tab:stage_ablation}
\end{threeparttable}
\end{table}

